Dimension-free Information Concentration via Exp-Concavity

Information concentration of probability measures have important implications in learning theory. Recently, it is discovered that the information content of a log-concave distribution concentrates around their differential entropy, albeit with an unpleasant dependence on the ambient dimension. In this work, we prove that if the potentials of the log-concave distribution are exp-concave, which is a central notion for fast rates in online and statistical learning, then the concentration of information can be further improved to depend only on the exp-concavity parameter, and hence, it can be dimension independent. Central to our proof is a novel yet simple application of the variance Brascamp-Lieb inequality. In the context of learning theory, our concentration-of-information result immediately implies high-probability results to many of the previous bounds that only hold in expectation.

==> APPsectionA.tex <==
\section*{Appendix B.}

\label{app:theorem}

% Note: in this sample, the section number is hard-coded in. Following
% proper LaTeX conventions, it should properly be coded as a reference:

%In this appendix we prove the following theorem from
%Section~\ref{sec:textree-generalization}:

In this appendix we finish the proof of \textbf{Theorem \ref{thm:BL_nonsmooth}} given \eqref{eq:transportation_cost_weak}. The proof is a suitable adaptation of the linearization procedure in \cite{cordero2017transport}.

Since continuous functions with compact support are dense in $L_2(\mu_{\tilde{V}})$, we will prove \textbf{Theorem \ref{thm:BL_nonsmooth}} for any continuous function with compact support. Notice that such functions are necessarily Lipschitz and hence differentiable $\mu_{\tilde{V}}$-almost everywhere. Since modifying $f$ in a set of $\mu_{\tilde{V}}$-measure 0 does not effect \eqref{eq:brascamp_lieb_nonsmooth}, we may henceforth assume that $f \in \mathcal{C}^1$ and has compact support. 



Since $V \in \C2$, $\nabla^2 V(y)$ is uniformly continuous on any compact set, and hence we have 
\beq \label{eq:hold12}
c_V(y+h,y) = \frac{1}{2} \ip{\nabla^2 V(y)h}{h} + \|h\|^2\cdot o(1)
\eeq
uniformly in $y$ on any compact set when $h\rightarrow 0$. Assume for the moment that $c_V(x,y) \geq \frac{\delta}{2}\|x-y\|^2$ for some $\delta >0$. Given any function $g \in \mathcal{C}^1$ with compact support and $\int g d\mu_{\tV} = 0$, introduce the infimal convolution associated with the cost $c_V$:
\beq \label{eq:inf_conv}
Q_c(g)(y) \coloneqq \inf_{x} \{ g(x) +  c_V(x,y)  \},
\eeq
whence $Q_c(g)(y) - g(x) \leq c_V(x,y).$ By the definition of $\calW_{c_{V}}$, for any joint probability measure $\pi$ having marginals $\mu_{\tV}$ and $\nu$, we must have
\beq
\calW_{c_{V}}(\mu_{\tV}, \nu) =  \inf_\pi \int c_V(x,y) d\pi(x,y) \geq \int Q_c(g) d\nu - \int g d\mu_{\tV}.
\eeq
Consider the infimum convolution of $\epsilon g$:
\beq  \label{eq:hold14}
Q_c(\epsilon g)(y) = \inf_x \{ \epsilon g(x) + c_V(x,y) \} = \inf_{h} \{\epsilon g(y+h) + c_V(y+h,y)  \}.
\eeq
Let $h_{\epsilon} = h_{\epsilon}(y)$ denote a point where the infimum is achieved. Since $g$ is globally Lipschitz, say with constant $L$, 
\begin{align}\label{eq:hold13}
\epsilon g(y+h_{\epsilon}) + c_{V}(y+h_{\epsilon},y) &\geq \epsilon g(y) - \epsilon L \|h_\epsilon\| + \delta\| h_{\epsilon} \|^2.
\end{align}On the other hand, by setting $h = 0$ in \eqref{eq:hold14}, we see that $\epsilon g(y+h_{\epsilon}) + c_{V}(y+h_{\epsilon},y) \leq \epsilon g(y)$. Combining this with \eqref{eq:hold13} gives
\beq \label{eq:h_is_order_eps}
\| h_\epsilon \| \leq \frac{L}{\delta} \epsilon.
\eeq
Notice that \eqref{eq:h_is_order_eps} does not depend on $y$, and hence $\| h_\epsilon \| = O(\epsilon)$ uniformly in $y$. 

As $g$ is compactly supported, we have $\sup |g| = M <\infty$. Let $\Omega$ be the support of $g$, and let $B_\epsilon \coloneqq \{ x \ | \ \exists y \in \Omega,   \| x - y \|^2 \leq \frac{2\epsilon M}{\delta} \}.$ We claim that $Q_c(\epsilon g) \geq 0$ on $B_\epsilon^c$. Indeed, for any $y \in B_\epsilon^c$, suppose that the infimum of $x$ in \eqref{eq:hold14} is attained in $\Omega$. Then $Q_c(\epsilon g) \geq    \frac{\delta}{2} \cdot \frac{2\epsilon M}{\delta}  -   \epsilon M = 0$, since $c_V(x,y) \geq \frac{\delta}{2}\|x-y\|^2$ and $\inf_{x\in \Omega}\|y-x\|^2\geq \frac{2\epsilon M}{\delta}$. On the other hand, if the infimum of $x$ in \eqref{eq:hold14} is attained outside $\Omega$, then $\epsilon g = 0$ and $c_V \geq 0$ implies that  $Q_c(\epsilon g) \geq 0$. 


For the sake of linearization, set $d\nu = 1+\epsilon f d\mu_{\tV}$ for some $f \in \mathcal{C}^1$ with $\int f d\mu_{\tV} = 0$. We now compute
\begin{align}
\calW_{c_{V}}(\mu_{\tV}, 1+\epsilon f d\mu_{\tV}) &\geq \int Q_c(\epsilon g) \l(1+\epsilon f\r)d\mu_{\tV}  &\textup{since } \int g d\mu_{\tV} = 0 \notag\\
&\geq \int_{B_\epsilon} Q_c(\epsilon g) \l(1+\epsilon f\r)d\mu_{\tV}  &\textup{since } Q_c(\epsilon g)  \geq 0 \textup{ on } B_\epsilon^c. \label{eq:W_versus_Qc}
\end{align}As the set $B_\epsilon$ is itself compact, we have, uniformly in $y$,
\begin{align}
 Q_c(\epsilon g)(y) &= \epsilon g(y+h_\epsilon) + c(y+h_\epsilon, y) \notag \\
&= \epsilon g(y) + \epsilon \ip{\nabla  g(y)}{h_\epsilon}  + \frac{1}{2} \ip{\nabla^2 V(y) h_\epsilon }{h_\epsilon}  + o(\epsilon^2)  \label{eq:hold15}
\end{align}where the last line follows by \eqref{eq:h_is_order_eps}. Noticing that \eqref{eq:hold15} is convex in $h_\epsilon$, we can find its minimum (up to $o(\epsilon^2)$) and write
\beq \label{eq:hold16}
 Q_c(\epsilon g)(y)  \geq \epsilon g(y) - \frac{\epsilon^2}{2}\ip{\nabla^2 V^{-1}(y) \nabla  g(y)}{\nabla  g(y)}  + o(\epsilon^2).
\eeq
Multiplying \eqref{eq:hold16} by $1+\epsilon f$ and integrate on $B_\epsilon$ w.r.t. $d\mu_{\tV}$, we get, using \eqref{eq:W_versus_Qc} and $\int f d\mu_{\tV} = \int g d\mu_{\tV} = 0$,
\begin{align}
\frac{1}{\epsilon^2} \calW_{c_{V}} \l(\mu_{\tV}, \l(1+\epsilon f \r) d\mu_{\tV} \r) \geq \int_{B_{\epsilon}} fgd\mu_{\tV} - \frac{1}{2} \int_{B_{\epsilon}} \ip{\nabla^2V^{-1}\nabla g}{\nabla g} d\mu_{\tV} + o(1). \label{eq:hold17}
\end{align}By definition, $B_\epsilon$ contains the support of $g$, and hence the integrals in \eqref{eq:hold17} are in fact over the whole space. We hence conclude
\beq \label{eq:hold18}
\liminf_{\epsilon \rightarrow 0} \frac{1}{\epsilon^2} \calW_{c_{V}} \l(\mu_{\tV}, \l(1+\epsilon f \r) d\mu_{\tV} \r) \geq \int_{} fgd\mu_{\tV} - \frac{1}{2} \int_{} \ip{\nabla^2V^{-1}\nabla g}{\nabla g} d\mu_{\tV}.
\eeq
Replacing $g$ by $\lambda g$ in \eqref{eq:hold18} and optimizing over $\lambda$, we get
\beq \label{eq:hold20}
\frac{ \l(\int fg d\mu_{\tV} \r)^2}{2\int \ip{\nabla V^{-1}\nabla g}{\nabla g}  d\mu_{\tV} } \leq \liminf_{\epsilon \rightarrow 0} \frac{1}{\epsilon^2} \calW_{c_{V}} \l(\mu_{\tV}, \l(1+\epsilon f \r) d\mu_{\tV} \r).  
\eeq

Moreover, using $\log(1+x) = x -\frac{x^2}{2}+ o(x^2)$ and $\int f d\mu_{\tV} = 0$, we can compute
\begin{align}
D\l(   \l(1+\epsilon f\r)d\mu_{\tV}  \|  \mu_{\tV} \r) &= \int \l(1+\epsilon f \r) \l(\epsilon f - \frac{\epsilon^2 f^2}{2}  + o(\epsilon^2) \r) d\mu_{\tV} \notag\\
&= \frac{\epsilon^2}{2} \int f^2 d\mu_{\tV} + o(\epsilon^2). \label{eq:hold19}
\end{align}

In the case of $c_V(x,y) \geq \frac{\delta}{2}\|x-y\|^2$, \textbf{Theorem \ref{thm:BL_nonsmooth}} then follows by using $g=f$ in \eqref{eq:hold20} and combing \eqref{eq:transportation_cost_weak} and \eqref{eq:hold19}. For general case, replace $V$ by $V+\frac{\delta\| \cdot \|^2}{2}$ and take $\delta \rightarrow 0$ in \eqref{eq:hold18} and \eqref{eq:hold19} to deduce the same inequalities.


==> prelim.tex <==
\section{Preliminaries}
Let $\mu$ be a probability measure having density $f$ (with respect to the Lebesgue measure) and let $X$ be the random variable associated with $\mu$. The differential entropy \cite{cover2012elements} of $X$ is defined as 
\beq \label{eq:diff_entropy}
h(\mu) = h(X) \coloneqq \EE_{\mu} [-\log f(X)].
\eeq The random variable $\tilde{h}(\mu) = \tilde{h}(X) \coloneqq -\log f(X)$ is called the \emph{information content} of $\mu$.


Throughout this paper, we consider probability measure of the form 
\beq
d\mu_V(x) \coloneqq \frac{e^{-V(x)}}{\int e^{-V}} dx, \label{eq:log-concave}
\eeq where $V$ is a convex function such that $\int e^{-V} < \infty$. For such measures, the concentration of differential entropy is the same as the concentration of the function $V$:
\begin{lemma}\label{lem:concentration_entropy=concentration_V}
Let $d\mu_V(x) \coloneqq \frac{e^{-V(x)}}{\int e^{-V}} dx$. We have $\PP\l( \left| V - \EE_{\mu_V} V \right| > t\r) = \PP\l( \left| \tilde{h}(\mu_V) - h(\mu_V) \right| > t\r)$ for all $t \in \RR$.
\end{lemma}

\begin{proof}
It suffices to notice that, for $X \sim d\mu_V$, 
\begin{align*}
\tilde{h}(\mu_V) - h(\mu_V) &= V(X) - \log \int e^{-V} - \l( \EE_{\mu_V} V - \log \int e^{-V} \r) \\
&= V - \EE_{\mu_V} V.
\end{align*}
\end{proof}

We henceforth focus on the quantity $\PP\l( \left| V - \EE_{\mu_V} V \right| > t\r)$.
%Hence, the concentration of information content for $d\mu_V$ is reduced t

Poincar\'{e} and exponential concentration for Lipschitz functions. 


Local norms.

Brascamp-Lieb inequality.

\begin{theorem}\emph{(Concentration of Information for Log-Concave Vectors)}
Let $d\mu_V(x) \coloneqq \frac{e^{-V(x)}}{\int e^{-V}} dx$ be a $d$-dimensional log-concave probability measure. Then 
\end{theorem}
